3D Reconstruction using Structured Light from off-the-shelf components

The coordinate measuring machine(CMM) has been the benchmark of accuracy in measuring solid objects from nearly past 50 years or more. However with the advent of 3D scanning technology, the accuracy and the density of point cloud generated has taken over. In this project we not only compare the different algorithms that can be used in a 3D scanning software, but also create our own 3D scanner from off-the-shelf components like camera and projector. Our objective has been : 1. To develop a prototype for 3D scanner to achieve a system that performs at optimal accuracy over a wide typology of objects. 2. To minimise the cost using off-the-shelf components. 3. To reach very close to the accuracy of CMM.

==> abbreviations.tex <==
\acsetup{first-style=short}

% class `abbrev': abbreviations:
\DeclareAcronym{ny}{
  short = NY ,
  long  = New York ,
  class = abbrev
}
\DeclareAcronym{la}{
  short = LA ,
  long  = Los Angeles ,
  class = abbrev
}
\DeclareAcronym{un}{
  short = UN ,
  long  = United Nations ,
  class = abbrev
}


==> declaration1.tex <==
\begin{titlepage}
\pagenumbering{empty}
\begin{center}
\Large\textsc{3D Reconstruction Using Structured Light}\\
\textsc{} \\
\small\textbf{\textsl{A project report submitted to}} \\
\small\textbf{\textsl{Visvesvaraya National Institute of Technology, Nagpur}} \\
\small\textbf{\textsl{in partial fulfillment of the requirements for the award of}} \\
\small\textbf{\textsl{the degree}} \\
\textsc{} \\
\Large\textbf{\text{BACHELOR OF TECHNOLOGY}}\\
\Large\textbf{\text{IN}}\\
\Large\textbf{\text{MECHANICAL ENGINEERING}}\\
\textsc{} \\
\textsl{by}\\
\textsc{} \\
\large{\textbf{Nachiket Jadhav}\hspace{35pt} \textbf{BT16EEE052}}\\
\large{\textbf{Aman Gajendra Jain} \hspace{30pt} \textbf{BT16EEE100}}\\

\textsc{} \\
\large\text{under the guidance of} \\
\textsc{} \\
\large{\textbf{Dr. Shital Chiddarwar}}\\
\textsc{} \\
\begin{figure}[h!]
\centering
\includegraphics[scale=1.5]{vnit_logo.png}
\end{figure}
\Large{\textbf{Department of Mechanical Engineering}}\\
\Large{\textbf{Visvesvaraya National Institute of Technology}}\\
\Large{\textbf{Nagpur 440 010(India)}}\\
\Large{\textbf{2020}}\\
% \small{\textcopyright} \small{Visvesvaraya National Institute of Technology (VNIT) 2019}

\textsc{} \\
\end{center}

\end{titlepage}

==> formatting.tex <==
\DeclareNameAlias{sortname}{last-first}
\DeclareFieldFormat{edition}{%
  \ifinteger{#1}
    {\ifnumequal{#1}{1}%
     {}%
     {\mkbibordedition{#1}~\bibstring{edition}}%
    }
    {#1\isdot}}

\DeclareFieldFormat[article,inbook,incollection]{title}{#1\isdot}
\DeclareFieldFormat[article,inbook,incollection]{citetitle}{#1\isdot}

\newrobustcmd{\MakeTitleCase}[1]{%
  \ifboolexpr{test {\ifentrytype{article}} or test {\ifentrytype{inbook}} or test {\ifentrytype{incollection}}}
    {#1}
    {\MakeSentenceCase{#1}}}

\DeclareFieldFormat{urldate}{\bibsentence\mkbibbrackets{\bibstring{urlseen}\space#1}}
\DeclareFieldFormat{url}{\bibstring{urlfrom}\addcolon\space\url{#1}}

\renewbibmacro*{journal}{%
  \iffieldundef{journaltitle}
    {}
    {\printtext[journaltitle]{%
       \printfield[titlecase]{journaltitle}%
       \setunit{\subtitlepunct}%
       \printfield[titlecase]{journalsubtitle}}
       \ifboolexpr{
         not test {\iffieldundef{url}}
         or
         not test {\iffieldundef{urldate}}
         or
         not test {\iffieldundef{doi}}
         or
         not test {\iffieldundef{eprint}}
       }
         {\nopunct\bibstring[\mkbibbrackets]{online}}%
         {}}}

\newbibmacro*{journal+issuetitle}{%
  \usebibmacro{journal}%
  \setunit*{\addspace}%
  \iffieldundef{series}
    {}
    {\newunit
     \printfield{series}%
     \setunit{\addspace}}%
  \newunit
  \usebibmacro{volume+number+eid}%
  \setunit{\addspace}%
  \usebibmacro{issue+date}%
  \setunit{\addcolon\space}%
  \usebibmacro{issue}%
  \newunit}

\NewBibliographyString{online}
\DefineBibliographyStrings{english}{%
  urlseen    = {accessed},
  online     = {online},
}
%\addbibresource{example.bib}
\renewcommand*{\nameyeardelim}{\addcomma\addspace}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}} % removes "In" preceeding journal title

==> weblinks.tex <==
\textbf{WEBLINKS}
\begin{enumerate}
    \item ugweb.cs.ualberta.ca/~vis/courses/robotics/lectures/Lec03MobileKin12.ppt
    \item https://www.theverge.com/2018/8/16/17693866/ford-self-driving-car-safety-report-dot
    \item https://www.micron.com/insight/on-the-road-to-full-autonomy-self-driving-cars-will-rely-on-ai-and-innovative-memory
    \item https://dewesoft.pro/online/course/pid-control
    \item https://spectrum.ieee.org/cars-that-think/transportation/self-driving/mit-experts-selfdriving-cars-wont-need-accurate-digital-maps
    \item https://www.tesla.com/autopilot
    \item https://www.kjronline.org/ViewImage.php?Type=F&aid=568151&id=F3&afn=68\_KJR\_18\_4\_570&fn=\_0068KJR
    \item https://towardsdatascience.com/applied-deep-learning-part-4-convolutional-neural-networks-584bc134c1e2
    \item https://www.analyticsvidhya.com/blog/2016/04/deep-learning-computer-vision-introduction-convolution-neural-networks/
    \item https://www.kdnuggets.com/2018/03/5-things-reinforcement-learning.html
    \item http://mi.eng.cam.ac.uk/~mg436/LectureSlides/MLSALT7/L6.pdf
    \item
\end{enumerate}


